Towards A Unified View of Sparse Feed-Forward Network in Pretraining Large Language Model

Large and sparse feed-forward layers (S-FFN) such as Mixture-of-Experts (MoE) have proven effective in scaling up Transformers model size for \textit{pretraining} large language models. By only activating part of the FFN parameters conditioning on input, S-FFN improves generalization performance while keeping training and inference costs (in FLOPs) fixed. In this work, we analyzed two major design choices of S-FFN: the memory block (a.k.a. expert) size and the memory block selection method under a general conceptual framework of sparse neural memory. Using this unified framework, we compare several S-FFN architectures for language modeling and provide insights into their relative efficacy and efficiency. We found a simpler selection method -- \textbf{\texttt{Avg-K}} that selects blocks through their mean aggregated hidden states, achieving lower perplexity in language model pretraining compared to existing MoE architectures including Switch Transformer (Fedus et al., 2021) and HashLayer (Roller et al., 2021).

==> 042_new_method.tex <==
\pdfoutput=1
\section{A new routing method --- \newMethod}
\label{sec:new_routing}
\input{table/new_method_compare}
% \vspace{-0.5em}
Shown by Fig. \ref{fig:355m_pareto}, a gated MoE has clear advantage over sparse memory. Basing on the contrastive analysis from \textsection\ref{sec:framework_analysis:selection}, we believe the current MoE already has a good design choice --- a reasonably large memory block size and a full-parameter key table. However, an important improvement is to make more use of each expert's key table for routing tokens. Additionally, it needs to be compute-efficient with smaller $g$ (\textsection\ref{sec:framework_analysis:granularity}).

To this end, we propose a new routing method --- \newMethod  --- as a hybrid design choice between sparse neural memory methods and mixture-of-experts methods. 

With \newMethod, we represent each block with the average of its key table $\mathbf{K}^{(i)} \in \mathbb{R}^{g \times d}$ along $g$-dimension --- $\mathbf{e}_i = \frac{1}{g} \sum_{j=0}^{g-1} \mathbf{k}^{(i)}_j = \texttt{\textbf{Avg}}(\mathbf{K}^{(i)}\texttt{,dim=0})$. Then, we use the dot product between $\mathbf{x}$ and the averages to select the top-$b$ selected block and route the token there for memory calculation (Eq. \ref{eq:ffn_memory}):
$$\mathbf{g}_i(\mathbf{x}) =
    \begin{cases}
      1 & i \in \left\{\text{top-}b \text{ of }[\mathbf{e}_0 , \cdots, \mathbf{e}_{B-1}] \cdot \mathbf{x}\right\} \\
      0 & \text{otherwise}
    \end{cases}\label{eq:new_method:route}$$
% \vspace{-1em}

Due to the linearity of averaging, the operation $\mathbf{e}_i \cdot \mathbf{x}$ is equivalent to calculating the average of dot products within a block without GeLU. Since all tokens share the averages, our method is efficient. We provide more rationale for our choice of average function in Appendix \ref{appendix:newMethod:rationale}.

Table \ref{tab:new_method:comparison} shows that the proposed \generalTerm design outperforms all other indirect methods.
With $<1\%$ additional FLOPs, \newMethod achieves 2.16 lower perplexity than \baseline(16.96), outperform \citep{switch_transformer} by 1.65 and \citep{hash_layer} by 0.5. % while Switch Transformer 0.51 lower and the best \hash 1.61 lower.
In Appendix \ref{appendix:newMethod:analysis}, we include a contrastive analysis with \oracle to understand the drastic improvement from block size $g=4096$ to $256$. 
% \vspace{-.5em}
\paragraph{Load balancing} Previously, load balancing has two-fold implication: \textbf{1)} to improve empirical training time \cite{switch_transformer}; \textbf{2)} more importantly, to prevent the expert representations from degeneration --- i.e. routing most tokens to a single expert \citep{first_modern_moe, factored_representation_moe}. Based on our observation, we hypothesize that load balancing is only \textit{optional} for \textit{learning} a good expert representation (i.e., the second implication) since our experiment with Switch enforces load balancing and experiment with \newMethod doesn't. And we further hypothesize that Switch's load balancing techniques will work for \newMethod due to our rationale in Appendix \ref{appendix:newMethod:analysis}. 
We also provide analysis for block usage (i.e. load balancing) for \newMethod in Appendix \ref{appendix:newMethod:load-balance}.
% Without load balancing constraints, \smoe with learned gate often degenerate to using only a handful of memory blocks (\textsection \ref{sec:bgd:moe}) while \newMethod does not suffer training instability. We found \newMethod uses blocks in a non-uniform fashion and varies across layers.
% Overall, \newMethod still matches Switch's performance with memory block size $g=4096$ or out-performs all other \smoe with memory block size $g\leq 256$. 
%We believe \newMethod is a better way to create block representations and leads to better $\mathbf{K}^g, \mathbf{V}^g$. 
% \vspace{-0.5em}
% \paragraph{Interpretability} \citet{key_value_memory} shows that rows of $\mathbf{K}$ of an end-to-end trained model strongly corresponds (i.e. by dot product) to human-interpretable --- surface- and semantic-level --- textual features. Since \newMethod heavily depends on dot products, their analysis could be easily extended for interpreting our model. In comparison, \hash is a lot harder to interpret due to random selection, and the relationship between $\mathbf{e}_i$ and $\mathbf{K}^{(i)}$ remains unclear for \switch or \smoe with conventional learned gate. 
% We defer such analysis to future work since this is beyond the scope of our paper.


% In addition to being conceptually \textit{simpler} and \textit{``naturally'' integrated}, our methods has the advantage of \textit{interpretability} over other indirect methods.
% With a larger block size $g=4096$, the perplexity of \newMethod matches that of \switch on out-of-domain. 
% \vspace{-0.5em}
% \paragraph{Simplicity}
% \paragraph{Load balancing} 
% \newMethod essentially applies a pooling over the chunked key table, whose cost is minuscule w.r.t., e.g., a conventionally-sized FFN even with $E=512$. In addition, this calculation could be parallelism by memory blocks on different devices. We believe this is a conceptually simpler and ``naturally'' integrated design than current methods, with load balancing constraints to be enforced (\textsection \ref{sec:bgd:moe}). For example, an iterative solver used for solving a constraint optimization problem \citep{base_layer} might get stuck in an infinite loop.
% \vspace{-.5em}
% \paragraph{Interpretability} 
%\section{Future work and Limitation}
%\vspace{-.5em}



% \leo{TODO: comparison with other MoE methods in new method section finish this paragraph}
% The additional pooling has negligible FLOPs cost, so the overall training budget is equivalent to Switch transformers. In addition to the pretraining objective (i.e. Causal Language Modeling objective), \citet{gshard, switch_transformer, glam} added a standard auxiliary loss, or, more recently,  \citet{base_layer} replace the loss with an equivalent linear assignment optimization to avoid inputs are processed by only a few blocks. In our experiments with \ref{fig:new_method:pareto}, we surprisingly found that without any auxiliary loss or optimization step our model performs competitively. When $g=4096$, \newMethod performs similarly to Switch and is outperformed by Hash on PILE. However, after we uses the observation that smaller block size improves performance, \newMethod quickly outperforms Hash and closely approach performance of Oracle with little (less than $1\%$ or even $0.5\%$) additional training FLOPs compared with a standard Dense baseline.

% \begin{figure}[th]
% \centering
%  \includegraphics[scale=0.6,trim={1em 1.3em 1em 1.1em},clip]{figs/avg-pool/pareto/avg-ppl.scatter+line.all_tasks.x=relative_total_flops_added.y=perplexity.In_OutOf-domain.pdf}
% \caption{Perplexity performance (lower the better) of all MoE methods in 355M ($E=16, k=4096$). \todo{Missing: Avg-K ($g=2048, 1024$), Hash($g=4096$)} This shows \newMethod closely approaches the performance of Oracle with little incurred cost, surpassing the best possible results from Hash($g=1$). \leo{TODO: convert this into a table and emphasize the minimal changes in flops}}
% \label{fig:new_method:pareto}
% \end{figure}



% Short list of finding 
% \begin{itemize}
%     \item \xian{Add double descent.}
%     \item Memory with smaller granularity is more immune against sparsity.
%     \item Memory with different selection method scales differently \xian{When we ``scale differently" people will expect results from models with varying magnitudes of size.} in sparsity: gating --- less sparse better; oracle --- optimal data;  \leo{how about we say ``different selection method has different sparsity behavior''?}  
 
% \end{itemize}


% We have gained some interesting insights on the both knobs given a fixed $k$. In this section, we want to come back to the end goal of our investigation --- ``sparsity''. Particularly, we want to study how the two knobs individually interplay with sparsity to inform future development of sparse memory. 

% \subsection{Sparsity $+$ Granularity}
% Following setup above $(d_m = 16 \cdot (4 \cdot d))$, we run a full sweep over $\left\{(g, k): g, k \in \{1, 64, 256, 1024, 2048, 4096\} \text{ and } g \leq k \right\}$ with \textbf{BOracle}. We also include $k=d_m$ to cover the extreme case. 

% In Fig \ref{fig:355m_sparsity+granularity}, we have the interesting observation that when granularity is smaller, the model performance is much more robust. Noticeably, given different granularity, the relationship between PPL and $k$ also changes. With $g < 256$, there's a ``double descent'' w.r.t. $k$, whereas the improvement seems monotonic for larger $g$.

% \begin{figure}[th]
% \centering
%  \includegraphics[scale=0.7]{figs/sparsity+granularity/avg-ppl.png}
%  % \caption{A single Oracle inserted with different $d_M = E \cdot d_m$}

% % \begin{subfigure}[b]{0.5\textwidth}
     
% %  \end{subfigure}
% % \centering
% % \caption{\leo{change subtitle in plot} Perplexity (lower the better) performance with . The error bar represent the variance of perplexity across different domains in PILE.}
% \caption{\leo{change subtitle in plot} \leo{Ingore $g > 4096$} Perplexity performance (lower the better)}
% \label{fig:355m_sparsity+granularity}
% \end{figure}

% \subsection{Sparsity $+$ Selection method}

% In this section, we include more selection methods to see if the pattern we observe could generalize across different selection methods. To this ends, we additionally consider two edge cases --- $g=1$ and $g=k$ because we are confident that observation in granularity will extrapolate to $1 < g < k$ in ceteris paribus settings.

% \paragraph{$g=k$ case} This is the largest possible granularity under our framework. We consider \textbf{Hash}, \textbf{Linear}, and \textbf{BOracle}. To our surprise, we found that the scaling behavior of selection methods are different. Given the same memory size and parameter, gating-based methods keep improving when the size of active memory increases. However, block representation with simple statistics (i.e. average) hit its limit around $k=4096$. Although Hash and Linear are not outperforming on PILE, they seems free of \textbf{BOracle}'s issue of double descent. Due to their intrinsic advantage in efficiency, this observation implies that a more sophisticated of block representation or mapping is needed to shift the current curve downward, approaching the row-wise \textbf{Oracle}. We also observe that \textbf{Hash} and \textbf{Linear} swap their ranking in validation set and PILE; this further shows the room of improvement of learned gating against its ``random'' baseline; and the lesson of comprehensive testing.

% \begin{figure}[th]
% \centering
%  \includegraphics[scale=0.7]{figs/sparsity+selection/g=k-avg-ppl.png}
%  % \caption{A single Oracle inserted with different $d_M = E \cdot d_m$}

% % \begin{subfigure}[b]{0.5\textwidth}
     
% %  \end{subfigure}
% % \centering
% % \caption{\leo{change subtitle in plot} Perplexity (lower the better) performance with . The error bar represent the variance of perplexity across different domains in PILE.}
% \caption{\leo{change subtitle in plot} \leo{Ingore $g > 4096$} Perplexity performance (lower the better) \leo{direct vs indirect behaviors are different}}
% \label{fig:355m_sparsity+selection:g=k}
% \end{figure}

% \paragraph{$g=1$ case} In this case, using \textbf{Linear} defeats the purpose of saving FLOPs because $\bm{\theta}$ will has the same size as $\mathbf{K}^{\mathcal{B}}$ and we could just use \textbf{Oracle}. Therefore, we only consider \textbf{Hash} and \textbf{BOracle}. \leo{Should we run PK-FFN with different $k$ as a proxy?} Similar to previous case, we also observe different scaling behavior from different selection methods, where \textbf{Oracle} has double descent and \textbf{Hash} does not. In addition, that one selection methods has advantage, by different margins, over another with different ks. \leo{potential logic loop: if we are saying Oracle has double descent, it seems any methods has to have similar behavior} 

% \begin{figure}[th]
% \centering
%  \includegraphics[scale=0.7]{figs/sparsity+selection/g=1-avg-ppl.png}
%  % \caption{A single Oracle inserted with different $d_M = E \cdot d_m$}

% % \begin{subfigure}[b]{0.5\textwidth}
     
% %  \end{subfigure}
% % \centering
% % \caption{\leo{change subtitle in plot} Perplexity (lower the better) performance with . The error bar represent the variance of perplexity across different domains in PILE.}
% \caption{\leo{change subtitle in plot} \leo{Ingore $g > 4096$} Perplexity performance (lower the better)}
% \label{fig:355m_sparsity+selection:g=1}
% \end{figure}


